sBelle Design Study Report

In this note, we compile results of various simulation studies for the upgrade of the Belle detector. Based on these studies, we propose a set of optimum or appropriate parameters of the detector.

==> KL.tex <==
 \section{$K_L$ reconstruction}
 \label{sec:klm}

\begin{figure}
 \begin{center}
  \includegraphics[width=0.85\textwidth]{epsfiles/kl/taunukl.eps}
  \caption{
  \label{fig:kl-taunu}
  The sensitivity dependence on the $K_L$ veto efficiency for the 
  $B\to\tau\nu$ decay.
  In the vertical axis is the luminosity ratio to achieve the same
  sensitivity and smaller is the better.
  }
 \end{center}
\end{figure}


==> author.fail.tex <==
\author{I.~Adachi
\thanks{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
\and
K.~Hara
\thanks{Nagoya University, Nagoya} % Nagoya
\and
T.~Hara
\thanks{Osaka University, Osaka} % Osaka
\and
T.~Higuchi
\thanks{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
\and
K.~Inami
\thanks{Nagoya University, Nagoya} % Nagoya
\and
H.~Ishino
\thanks{Tokyo Institute of Technology, Tokyo} % TIT
\and
N.~Katayama
\thanks{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
\and
T.~Karim
\thanks{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
\and
T.~Kawasaki
\thanks{Niigata University, Niigata} % Niigata
\and
A.~Kibayashi
\thanks{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
\and
P.~Kri\v zan
\thanks{University of Ljubljana, Ljubljana}
\and
\thanks{J. Stefan Institute, Ljubljana} % Ljubljana
P.~Krokovny
\and
\thanks{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
Y.~Kuroki
\and
\thanks{Osaka University, Osaka} % Osaka
A.~Kuzmin
\and
\thanks{Budker Institute of Nuclear Physics, Novosibirsk} % BINP
\and
I.~Nakamura
\thanks{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
\and
M.~Nakao
\thanks{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
\and
S.~Nishida
\thanks{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
\and
H.~Ozaki
\thanks{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
\and
R.~Pestotnik
\thanks{J. Stefan Institute, Ljubljana} % Ljubljana
\and
Y.~Sakai
\thanks{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
\and
C.~Schwanda
\thanks{Institute of High Energy Physics, Vienna} % Vienna
\and
S.~Shinomiya
\thanks{Osaka University, Osaka} % Osaka
\and
K.~Sumisawa
\thanks{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
\and
O.~Tajima
\thanks{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
\and
T.~Tsuboyama
\thanks{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
\and
Y.~Ushiroda
\thanks{High Energy Accelerator Research Organization (KEK), Tsukuba} % KEK
}

